Towards Equitable ASD Diagnostics: A Comparative Study of Machine and Deep Learning Models Using Behavioral and Facial Data

Autism Spectrum Disorder (ASD) is often underdiagnosed in females due to gender-specific symptom differences overlooked by conventional diagnostics. This study evaluates machine learning models, particularly Random Forest and convolutional neural networks, for enhancing ASD diagnosis through structured data and facial image analysis. Random Forest achieved 100% validation accuracy across datasets, highlighting its ability to manage complex relationships and reduce false negatives, which is crucial for early intervention and addressing gender biases. In image-based analysis, MobileNet outperformed the baseline CNN, achieving 87% accuracy, though a 30% validation loss suggests possible overfitting, requiring further optimization for robustness in clinical settings. Future work will emphasize hyperparameter tuning, regularization, and transfer learning. Integrating behavioral data with facial analysis could improve diagnosis for underdiagnosed groups. These findings suggest Random Forest's high accuracy and balanced precision-recall metrics could enhance clinical workflows. MobileNet's lightweight structure also shows promise for resource-limited environments, enabling accessible ASD screening. Addressing model explainability and clinician trust will be vital.

==> comments.tex <==
For the Related Works section that needs to be created from scratch, it would be beneficial to identify and discuss recent articles on Antimicrobial Resistance (AMR) Detection, especially those that focus on Leveraging Whole Genome Sequencing and Machine Learning. This section should emphasize the limitations and weaknesses of existing and state-of-the-art approaches, which will help lay a strong foundation for our contributions.

 
-------------------
In the Proposed Method section, I suggest including one or more figures to visualize the implementation architecture. This section could be structured into phases such as:

Collecting and preprocessing datasets
Selecting ML models, with justifications for each choice
Discussing the challenges encountered during the study (e.g., overfitting, underfitting)
Evaluating and optimizing the models, with clear explanations for the decisions made

--> Undone: leave the current section as is. I don't see a need to restructure it as mentioned here.
------------------------

For the Results and Discussion section, I recommend creating and adding new plots to visually represent some of the data currently presented in tables. Bar and pie charts could effectively highlight the key findings and make the information more accessible to readers.
---> done
 
------------------
Additionally, the Introduction section could be strengthened by incorporating statistics on AMR, such as the number of cases each year, projected future figures, and the economic and societal costs associated with the issue. This would provide a compelling case for the importance of early detection and highlight the significant role that machine learning can play in addressing these challenges. 
---> Done

New comments: by Rahouti:
- Figs highlighted in red are not referenced in the text 
- Table 4 must be rechecked. Some values are bigger than 1 (100\%)
- All sections were grammatically checked, except section 3 (methodology)

==> venues.tex <==
- Journal of Biomedical Informatics, Elsevier. IF 4. Review Time 58 days.

- International Journal of Medical Informatics, Elsevier. IF 3.7. Review Time 66 days.

- Computer Methods and Programs in Biomedicine, Elsevier. IF 5. Review Time 90 days.

- Journal of Autism and Developmental Disorders, Springer. IF 3.5. Selected for submission

- Health Information Science and Systems, Springer. IF 4.7

- Journal of Medical Systems, Springer. IF 3.5.

- Medical \& Biological Engineering \& Computing, Springer. IF 2.6

- Pattern Analysis and Applications, Springer. IF 3.7

- Artificial Intelligence in Medicine, Elsevier. IF 6.1

- ACM Transactions on Intelligent Systems and Technology.

- ACM Transactions on Multimedia Computing, Communications, and Applications

- Neural Computing and Applications, Springer. IF 4.5

- Journal of Medical and Biological Engineering, Springer. IF 1.6

- Cognitive Computation, Springer. IF 4.3

- Neurocomputing, Elsevier. IF 5.5. Review Time 81 days.

- Review Journal of Autism and Developmental Disorders, Springer. IF 2.9. Rejected

- Autism: The International Journal of Research and Practice (Sage). IF 5.5.
Autism: The International Journal of Research and Practice

- Journal of Medical Internet Research, IF 6. Q1 Journal
Journal of Medical Internet Research (JMIR)

Frontiers in Psychiatry (Autism Spectrum Disorders Section)

